TiVaT: A Transformer with a Single Unified Mechanism for Capturing Asynchronous Dependencies in Multivariate Time Series Forecasting

Multivariate time series (MTS) forecasting is vital across various domains but remains challenging due to the need to simultaneously model temporal and inter-variate dependencies. Existing channel-dependent models, where Transformer-based models dominate, process these dependencies separately, limiting their capacity to capture complex interactions such as lead-lag dynamics. To address this issue, we propose TiVaT (Time-variate Transformer), a novel architecture incorporating a single unified module, a Joint-Axis (JA) attention module, that concurrently processes temporal and variate modeling. The JA attention module dynamically selects relevant features to particularly capture asynchronous interactions. In addition, we introduce distance-aware time-variate sampling in the JA attention, a novel mechanism that extracts significant patterns through a learned 2D embedding space while reducing noise. Extensive experiments demonstrate TiVaT's overall performance across diverse datasets, particularly excelling in scenarios with intricate asynchronous dependencies.

==> table/cfg.tex <==

\begin{table}[h]
\caption{Model configurations of TiVaT}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccccccccc}
\hline
             & Num blocks &Patch&Stride & Model dim & FFN dim & Learning rate & Per$_{\Delta_{t}}$ &  Per$_{\Delta_{v}}$&  Num $R_q^{self}$ &Num $R_q$  \\             
\hline
ECL          &     3   &  16&8      &   512         &    512       &   0.0005         & 0.2           &      0.2    &40 &40    \\
ETTh1        &     2   &8   &4      &     128       &   1024       &    0.0001        &  0.2          &   0.2       &40 &20     \\
ETTh2        &       2 &8   &4      &      128      &   256        &     0.0001       &      0.6      &     0.4     &20 &20         \\
ETTm1        &     2   &8   &4      &     128       &   1024       &      0.0001      &  0.6          &     0.2     &40 &40        \\
ETTm2        &       2 &8   &4      &      128      &   256        &      0.0001      & 0.2           &      0.2    &20 &40     \\
Exchange     &      2  & 8  &4      &       128     &   256        &      0.0001      &      0.2      &    0.2      &40 &40     \\
Traffic      &     4   &16  &8      &  128          &   512        &       0.001      &      0.1      &     0.2     &40 &40       \\
Weather      &    3    &16  &8      &     512       &   1024       &      0.0001      &        0.4    &      0.8    &40 &40     \\
\hline
\end{tabular}
}
\label{tbl:cfg}
\end{table}

==> table/sub.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \renewcommand{\arraystretch}{} 
% \begin{table*}[h]
% \large  
% \caption{Results for long-term forecasting. The reported values are averaged over four different prediction horizons: \{96, 192, 336, 720\}. Lower MSE or MAE values indicate better predictive performance. The input sequence length is fixed at 96 across all experiments.}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \hline
% \multicolumn{1}{c|}{\multirow{2}{*}{Models}} & \multicolumn{2}{c|}{\textbf{TiVaT}} & \multicolumn{2}{c|}{iTransformer} & \multicolumn{2}{c|}{CARD} & \multicolumn{2}{c|}{TimeMixer} & \multicolumn{2}{c|}{ModernTCN} & \multicolumn{2}{c|}{Crossformer}   & \multicolumn{2}{c|}{PatchTST}
%  & \multicolumn{2}{c|}{TimesNet} & \multicolumn{2}{c}{DLinear}  \\ 
% \multicolumn{1}{c|}{} & \multicolumn{2}{c|}{\textbf{(Ours)}}& \multicolumn{2}{c|}{(2024)} & \multicolumn{2}{c|}{(2024)} & \multicolumn{2}{c|}{(2024)} &\multicolumn{2}{c|}{(2024)}  & \multicolumn{2}{c|}{(2023)}&\multicolumn{2}{c|}{(2023)} & \multicolumn{2}{c|}{(2023)}&\multicolumn{2}{c}{(2023)} \\ \cline{2-19} 

% \multicolumn{1}{c|}{Metric} & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE& MSE & MAE & MSE & MAE  \\ \hline\hline

% ETTh1      & \textbf{\textcolor{red}{0.434}} & 0.435 & 0.454 & 0.447 & 0.442 & \textbf{\textcolor{red}{0.429}} & 0.447 & 0.440 &{\textbf{\textcolor{blue}{0.435}}} &{\textbf{\textcolor{blue}{0.431}}} & 0.529 & 0.522&0.469&0.454 & 0.458 & 0.450        & 0.456                   & 0.452      \\ %\hline
% ETTh2      & 0.374 & 0.412 & 0.383 & 0.407 & 0.368 & {\textbf{\textcolor{blue}}{0.390}}&{\textbf{\textcolor{blue}{0.364}}} & 0.395 & \textbf{\textcolor{red}{0.354}}  & \textbf{\textcolor{red}{0.388}}  & 0.942 & 0.684 &0.387&0.407& 0.414                   & 0.427                   & 0.559                   & 0.515\\ %\hline
% ETTm1      & {\textbf{\textcolor{blue}{0.382}}} & 0.397 & 0.407 & 0.410 & 0.383& 0.383 & \textbf{\textcolor{red}{0.381}} & {\textbf{\textcolor{blue}{0.395}}} & 0.386 & 0.400 & 0.513 & 0.496&0.387&0.400 & 0.400                   & 0.406                   & 0.403                   & 0.407 \\ %\hline
% ETTm2      & 0.278 & 0.325 & 0.288 & 0.332 & \textbf{\textcolor{red}{0.271}} & \textbf{\textcolor{red}{0.316}}& {\textbf{\textcolor{blue}{0.275}}} & {\textbf{\textcolor{blue}{0.323}}} & 0.279 & {\textbf{\textcolor{blue}{0.323}}} & 0.757 & 0.610 &0.281&0.326 & 0.291                   & 0.333                   & 0.350                   & 0.401     \\ %\hline
% Exchange   & \textbf{\textcolor{red}{0.349}} & \textbf{\textcolor{red}{0.398}}& 0.360     & {\textbf{\textcolor{blue}{0.403}}}   & 0.369 & 0.409 & 0.397 & 0.414 & {\textbf{\textcolor{blue}{0.354}}}   &  0.419 & 0.940 & 0.707 &0.367&0.404& 0.416                   & 0.443                   & 0.353                   & 0.414                \\ %\hline
% ECL        & \textbf{\textcolor{red}{0.166}} & {\textbf{\textcolor{blue}{0.262}}} & 0.178 & 0.270 & {\textbf{\textcolor{blue}{0.169}}} & \textbf{\textcolor{red}{0.258}} & 0.182 & 0.272 & 0.205 & 0.287 & 0.244 & 0.334 & 0.205 & 0.290  & 0.168                   & 0.272                   & 0.197                   & 0.282        \\ %\hline
% Traffic   & {\textbf{\textcolor{blue}{0.430}}} & 0.299 & \textbf{\textcolor{red}{0.428}}     & \textbf{\textcolor{red}{0.282} }    & 0.453 & \textbf{\textcolor{red}{0.282}} & 0.484 & 
%  {\textbf{\textcolor{blue}{0.297}}}  & 0.626  & 0.378  & 0.550 & 0.304 &0.481&0.304 & 0.620                   & 0.336                   & 0.625                   & 0.383            \\ %\hline
% Weather    & {\textbf{\textcolor{blue}{0.240}}} & {\textbf{\textcolor{blue}{0.270}}} & 0.258 & 0.278 & \textbf{\textcolor{red}{0.239}} &\textbf{\textcolor{red}{0.261}}& 0.240 & 0.271 & {\textbf{\textcolor{blue}{0.240}}} & 0.273 & 0.259 & 0.315 &0.259 &0.281 & 0.172                   & 0.220                   & 0.196                   & 0.255   \\ \hline

% \end{tabular}
% }
% \label{tbl:main_results}
% \end{table*}

\renewcommand{\arraystretch}{} 
\begin{table*}[t!]
\large  
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c|cc|cc|cc|cc|cc|cc|cc|cc|cc}
% \hline
% \multirow{2}{*}{Models} & \multicolumn{2}{c|}{\textbf{TiVaT}} & \multicolumn{2}{c|}{DeformableTST} & \multicolumn{2}{c|}{TimeXer} & \multicolumn{2}{c|}{TimeMixer} & \multicolumn{2}{c|}{iTransformer} & \multicolumn{2}{c|}{VCformer} & \multicolumn{2}{c|}{PatchTST} & \multicolumn{2}{c|}{TimesNet} & \multicolumn{2}{c}{DLinear} \\
%                         & \multicolumn{2}{c|}{\textbf{(Ours)}}  & \multicolumn{2}{c|}{(2024)}          & \multicolumn{2}{c|}{(2024)}    & \multicolumn{2}{c|}{(2024)}      & \multicolumn{2}{c|}{(2024)}         & \multicolumn{2}{c|}{(2024)}     & \multicolumn{2}{c|}{(2023)}     & \multicolumn{2}{c|}{(2023)}     & \multicolumn{2}{c}{(2023)}    \\ 
% \hline
% Metric                  & MSE              & MAE              & MSE              & MAE             & MSE           & MAE          & MSE            & MAE           & MSE             & MAE             & MSE           & MAE           & MSE           & MAE           & MSE           & MAE           & MSE          & MAE          \\ \hline
% ETTh1                   & \textbf{\textcolor{blue}{{0.434}}}            & \textbf{\textcolor{blue}{{0.435}}}            & \textbf{\textcolor{red}{0.425}}            & \textbf{\textcolor{red}{0.428}}           & 0.437         & 0.437        & 0.447          & 0.440         & 0.454           & 0.447           & 0.529         & 0.522         & 0.469         & 0.454         & 0.458         & 0.450         & 0.456        & 0.452        \\
% ETTh2                   & 0.374            & 0.412            & \textbf{\textcolor{red}{0.346}}            & \textbf{\textcolor{red}{0.382}}           & 0.367         & 0.396        & \textbf{\textcolor{blue}{{0.364}}}          & \textbf{\textcolor{blue}{{0.395}}}         & 0.383           & 0.407           & 0.942         & 0.684         & 0.387         & 0.407         & 0.414         & 0.427         & 0.559        & 0.515        \\
% ETTm1                   & 0.382            & \textbf{\textcolor{blue}{{0.397}}}            & \textbf{\textcolor{red}{0.373}}            & \textbf{\textcolor{red}{0.395}}           & 0.382         & \textbf{\textcolor{blue}{{0.397}}}        & \textbf{\textcolor{blue}{{0.381}}}          & \textbf{\textcolor{red}{0.395}}         & 0.407           & 0.410           & 0.513         & 0.496         & 0.387         & 0.400         & 0.400         & 0.406         & 0.403        & 0.407        \\
% ETTm2                   & 0.278            & 0.325            & 0.283            & 0.327           & \textbf{\textcolor{red}{0.274}}         & \textbf{\textcolor{red}{0.322}}        & \textbf{\textcolor{blue}{{0.275}}}          & \textbf{\textcolor{blue}{{0.323}}}         & 0.288           & 0.332           & 0.757         & 0.610         & 0.281         & 0.326         & 0.291         & 0.333         & 0.350        & 0.401        \\
% Exchange                & \textbf{\textcolor{red}{0.349}}            & \textbf{\textcolor{red}{0.398}}            & 0.375            & 0.418           & 0.422         & 0.416        & 0.397          & 0.414         & 0.360           & \textbf{\textcolor{blue}{{0.403}}}           & 0.940         & 0.707         & 0.367         & 0.404         & 0.416         & 0.443         & \textbf{\textcolor{blue}{{0.353}}}      & 0.414        \\
% ECL                     & \textbf{\textcolor{red}{0.166}}            & \textbf{\textcolor{red}{0.262}}            & 0.183            & 0.278           & 0.171         & \textbf{\textcolor{blue}{{0.270}}}        & 0.182          & 0.272         & 0.178           & \textbf{\textcolor{blue}{{0.270}}}           & 0.244         & 0.334         & 0.205         & 0.290         & \textbf{\textcolor{blue}{{0.168}}}         & 0.272         & 0.197        & 0.282        \\
% Traffic                 & \textbf{\textcolor{blue}{{0.438}}}            & 0.298            & 0.445            & \textbf{\textcolor{blue}{{0.285}}}           & 0.466         & 0.287        & 0.484          & 0.297         & \textbf{\textcolor{red}{0.428}}           & \textbf{\textcolor{red}{0.282}}           & 0.550         & 0.304         & 0.481         & 0.304         & 0.620         & 0.336         & 0.625        & 0.383        \\
% Weather                 & \textbf{\textcolor{red}{{0.240}}}            & \textbf{\textcolor{red}{0.270}}            & 0.251            & 0.276           & \textbf{\textcolor{blue}{{0.241}}}         & \textbf{\textcolor{blue}{{0.271}}}        & \textbf{\textcolor{red}{0.240}}          & \textbf{\textcolor{blue}{{0.271}}}         & 0.258           & 0.278           & 0.259         & 0.315         & 0.259         & 0.281         & 0.259         & 0.287         & 0.265        & 0.317        \\ \hline
% \end{tabular}%
% }
\begin{tabular}{c|cccccccccccccccccc}
\toprule
Types                         & \multicolumn{10}{c|}{Channel Dependent Models}                                                                                                                                                                  & \multicolumn{8}{c}{Channel Independent Models}                                                                                             \\ \midrule
\multicolumn{1}{c|}{Models}   & \multicolumn{2}{c|}{\textbf{TiVaT}} & \multicolumn{2}{c|}{TimeXer}       & \multicolumn{2}{c|}{VCformer}                             & \multicolumn{2}{c|}{DeformableTST} & \multicolumn{2}{c|}{iTransformer}  & \multicolumn{2}{c|}{TimeMixer}     & \multicolumn{2}{c|}{PatchTST}      & \multicolumn{2}{c|}{TimesNet}      & \multicolumn{2}{c}{DLinear} \\
\multicolumn{1}{c|}{}         & \multicolumn{2}{c|}{\textbf{Ours}}  & \multicolumn{2}{c|}{(2024)}          & \multicolumn{2}{c|}{(2024)}                                 & \multicolumn{2}{c|}{(2024)}          & \multicolumn{2}{c|}{(2024)}          & \multicolumn{2}{c|}{(2024)}          & \multicolumn{2}{c|}{(2023)}          & \multicolumn{2}{c|}{(2023)}          & \multicolumn{2}{c}{(2023)}    \\ \midrule
\multicolumn{1}{c|}{Metrics}   & MSE    & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}                          & MSE   & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}   & MSE   & \multicolumn{1}{c|}{MAE}   & MSE          & MAE          \\ \midrule
\multicolumn{1}{c|}{ETTh1}    & \textcolor{blue}{0.434}  & \multicolumn{1}{c|}{\textcolor{blue}{0.435}} & 0.437 & \multicolumn{1}{c|}{0.437} & 0.439 & \multicolumn{1}{c|}{0.437}                        & \textcolor{red}{0.425} & \multicolumn{1}{c|}{\textcolor{red}{0.428}} & 0.454 & \multicolumn{1}{c|}{0.447} & 0.447 & \multicolumn{1}{c|}{0.440} & 0.469 & \multicolumn{1}{c|}{0.454} & 0.458 & \multicolumn{1}{c|}{0.450} & 0.456        & 0.452        \\
\multicolumn{1}{c|}{ETTh2}    & 0.374  & \multicolumn{1}{c|}{0.412} & 0.367 & \multicolumn{1}{c|}{0.396} & 0.377 & \multicolumn{1}{c|}{0.403}                        & \textcolor{red}{0.346} & \multicolumn{1}{c|}{\textcolor{red}{0.382}} & 0.383 & \multicolumn{1}{c|}{0.407} & \textcolor{blue}{0.364} & \multicolumn{1}{c|}{\textcolor{blue}{0.395}} & 0.387 & \multicolumn{1}{c|}{0.407} & 0.414 & \multicolumn{1}{c|}{0.427} & 0.559        & 0.515        \\
\multicolumn{1}{c|}{ETTm1}    & \textcolor{blue}{0.381}  & \multicolumn{1}{c|}{\textcolor{blue}{0.397}} & 0.382 & \multicolumn{1}{c|}{\textcolor{blue}{0.397}} & 0.387 & \multicolumn{1}{c|}{\textcolor{blue}{0.397}}                        & \textcolor{red}{0.373} & \multicolumn{1}{c|}{\textcolor{red}{0.395}} & 0.407 & \multicolumn{1}{c|}{0.410} & \textcolor{blue}{0.381} & \multicolumn{1}{c|}{\textcolor{red}{0.395}} & 0.387 & \multicolumn{1}{c|}{0.400} & 0.400 & \multicolumn{1}{c|}{0.406} & 0.403        & 0.407        \\
\multicolumn{1}{c|}{ETTm2}    & 0.278  & \multicolumn{1}{c|}{0.325} & \textcolor{red}{0.274} & \multicolumn{1}{c|}{\textcolor{red}{0.322}} & 0.285 & \multicolumn{1}{c|}{0.330}                        & 0.283 & \multicolumn{1}{c|}{0.327} & 0.288 & \multicolumn{1}{c|}{0.332} & \textcolor{blue}{0.275} & \multicolumn{1}{c|}{\textcolor{blue}{0.323}} & 0.281 & \multicolumn{1}{c|}{0.326} & 0.291 & \multicolumn{1}{c|}{0.333} & 0.350        & 0.401        \\
\multicolumn{1}{c|}{Exchange} & \textcolor{red}{0.349}  & \multicolumn{1}{c|}{\textcolor{red}{0.398}} & 0.422 & \multicolumn{1}{c|}{0.416} & 0.355 & \multicolumn{1}{c|}{\textcolor{blue}{0.402}} & 0.375 & \multicolumn{1}{c|}{0.418} & 0.360 & \multicolumn{1}{c|}{0.403} & 0.397 & \multicolumn{1}{c|}{0.414} & 0.367 & \multicolumn{1}{c|}{0.404} & 0.416 & \multicolumn{1}{c|}{0.443} & \textcolor{blue}{0.353}        & 0.414        \\
\multicolumn{1}{c|}{Weather}  & \textcolor{red}{0.240}  & \multicolumn{1}{c|}{\textcolor{red}{0.270}} & \textcolor{blue}{0.241} & \multicolumn{1}{c|}{\textcolor{blue}{0.271}} & 0.258 & \multicolumn{1}{c|}{0.282}                        & 0.251 & \multicolumn{1}{c|}{0.276} & 0.258 & \multicolumn{1}{c|}{0.278} & \textcolor{red}{0.240} & \multicolumn{1}{c|}{\textcolor{blue}{0.271}} & 0.259 & \multicolumn{1}{c|}{0.281} & 0.259 & \multicolumn{1}{c|}{0.287} & 0.265        & 0.317        \\
\multicolumn{1}{c|}{ECL}      & \textcolor{red}{0.166}  & \multicolumn{1}{c|}{\textcolor{red}{0.262}} & 0.171 & \multicolumn{1}{c|}{0.270} & 0.180 & \multicolumn{1}{c|}{\textcolor{blue}{0.267}} & 0.183 & \multicolumn{1}{c|}{0.278} & 0.178 & \multicolumn{1}{c|}{0.270} & 0.182 & \multicolumn{1}{c|}{0.272} & 0.205 & \multicolumn{1}{c|}{0.290} & \textcolor{blue}{0.168} & \multicolumn{1}{c|}{0.272} & 0.197        & 0.282        \\
\multicolumn{1}{c|}{Traffic}  & \textcolor{blue}{0.438}  & \multicolumn{1}{c|}{0.298} & 0.466 & \multicolumn{1}{c|}{0.287} & 0.550 & \multicolumn{1}{c|}{0.304}                        & 0.445 & \multicolumn{1}{c|}{\textcolor{blue}{0.285}} & \textcolor{red}{0.428} & \multicolumn{1}{c|}{\textcolor{red}{0.282}} & 0.484 & \multicolumn{1}{c|}{0.297} & 0.481 & \multicolumn{1}{c|}{0.304} & 0.620 & \multicolumn{1}{c|}{0.336} & 0.625        & 0.383       \\ \bottomrule
\end{tabular}%
}
\caption{Results for long-term forecasting.}
\label{tbl:main_results}
\end{table*}
